Efficient Complex Event Processing in Information-centric Networking at the Edge

Information-centric Networking (ICN) is an emerging Internet architecture that offers promising features, such as in-network caching and named data addressing, to support the edge computing paradigm, in particular Internet-of-Things (IoT) applications. ICN can benefit from Complex Event Processing (CEP), which is an in-network processing paradigm to specify and perform efficient query operations on data streams. However, integrating CEP into ICN is a challenging task due to the following reasons: (1) typical ICN architectures do not provide support for forwarding and processing continuous data streams; (2) IoT applications often need short response times and require robust event detection, which both are hard to accomplish using existing CEP systems. In this article, we present a novel network architecture, called INetCEP, for efficient CEP-based in-network processing as part of ICN. INetCEP enables efficient data processing in ICN by means of (1) a unified communication model that supports continuous data streams, (2) a meta query language for CEP to specify data processing operations in the data plane, and (3) query processing algorithms to resolve the specified operations. Our experimental results for two IoT use cases and datasets show that INetCEP offers very short response times of up to 73 {\mu}s under high workload and is more than 15X faster in terms of forwarding events than the state-of-the-art CEP system Flink. Furthermore, the delivery and processing of complex queries is around 32X faster than Flink and more than 100X faster than a naive pull-based reference approach, while maintaining 100% accuracy.

==> sections/systemmodel.tex <==


 \begin{comment}
\begin{figure}[t]
	\centering
	\includegraphics[width=\linewidth]{figures/pdfs/Consumer-initiated_INetCEP.pdf}
	\setlength{\abovecaptionskip}{0pt}
	%\setlength{\belowcaptionskip}{-17pt}
	\caption{\added{\system communication model supports pull-based communication and fetches latest \Data packet.}}
	\label{fig:inetcep_pull}
\end{figure}

 
 \begin{figure}[t]
	\centering
	\includegraphics[width=\linewidth]{figures/pdfs/Producer-initiated_INetCEP.pdf}
	\setlength{\abovecaptionskip}{0pt}
	%\setlength{\belowcaptionskip}{-17pt}
	\caption{\added{\system communication model supports push-based communication without creating endless \ac{PIT} entries.}}
	\label{fig:inetcep_push}
\end{figure}



\begin{table}[]
\small
\begin{tabular}{ll}
\hline
Notation & Meaning \\
\hline
  $qi$       &  query interest   \\
  $q$       &  a CEP query   \\
  $D$       &  Continuous data stream   \\        
  $G$       &  Operator graph           \\
  $\Omega$  &   Set of CEP operators ($\omega \in \Omega$)  \\
  $f_\omega$ &  processing logic of an operator  \\
  $\Omega_{UD}$ & Set of user-defined operators ($\omega_{UD} \in \Omega_{UD}$)  \\
  $N$       &  Set of nodes ($n \in N$) \\
  $NM_{n}$ & Node manager for each node $n$  \\
  $E$       & Set of events $(e \in E)$ \\
  $f_{\omega}$  &   Processing logic of an operator \\
  $C_{\omega}$  &   Operator container \\
  $eq_{\omega_{UD}}$ &  Event queue for each $\omega_{UD}$  \\
  $b_s$ and $b_r$   &   Sent and received batch of events  \\
  $t_{backoff}$ & Queue polling backoff time \\
\hline
\end{tabular}
\setlength{\abovecaptionskip}{0pt}
\setlength{\belowcaptionskip}{-5pt}
\caption{Notations and their meaning.}
\label{tab:notations}
\end{table}
\end{comment}

\section{The \system Architecture}\label{sec:designl}

Every \ac{CCN} node can act either as a \emph{producer}, a \emph{consumer} or a \emph{broker}. \added{A \ac{CCN} node here refers a system entity that complies to the \ac{CCN} protocol as explained in \Cref{sec:preliminaries}. A CCN broker} is an in-network element, i.e., an \system aware \ac{CCN} router, while a producer or consumer is an end device, \eg a sensor or a mobile device. 
On the one hand, consumers can request a specific data item using an \Interest packet, where brokers forward the request received by consumers to support request-reply interaction, as illustrated in \Cref{fig:inetcep} on the left.
%\circled{2}
The producer replies with a data object contained in a \Data packet.
On the other hand, brokers process an unbounded and ordered \emph{data streams} generated by producers, which happens as illustrated in \Cref{fig:inetcep} on the right and is explained below.
%Consumer registers with an asynchronous query interest $qi$, but also can request data using a \ac{CCN} \Interest packet (cf. \Cref{fig:inetcep_push}).

\begin{table}[]
%\footnotesize
\scriptsize
    \centering
    \begin{tabular}{ll}%p{5cm}}
    \toprule
        Packet Type code & Packet Type  \\%& Packet Description  \\
        \midrule
        0x00             & \Interest     \\%& Interest packet to express a request on a data object. \\
        0x01             & \Data         \\%& Data packet to satisfy a request expressed by an Interest. \\
        0x02             & \AddQInterest \\%& Add Query Interest packet to express query on a data object \\
        0x03             & \RmQInterest  \\%& Remove Query Interest packet to remove query on a data object \\
        0x04             & \DataStream  \\%& Data Stream packet representing continuous time series data. \\
        \bottomrule
    \end{tabular}
    \caption{\added{Packet Types}}
    \label{tab:pak_types}
\end{table}

\begin{table*}
%\footnotesize
\scriptsize
\begin{tabular}{|p{2cm}|lp{4cm}|p{2cm}p{6cm}|}
\hline
\multirow{2}{*}{\textbf{Characteristic}}            & \multicolumn{2}{c|}{\textbf{Old Architecture}}                                       & \multicolumn{2}{c|}{\textbf{Our Architecture}}                                                                     \\  
                                 & \ac{ICN} & Description                                     & \system           & Description                                                            \\ \hline
\multirow{5}{*}{\begin{minipage}{1.5cm}Packet Types (cf. \S\ref{subsubsec:handling})\end{minipage}}      & \Interest  & {Interest packet to express a request on a data object}                                & \Interest         & {Interest packet to express a request on a data object}    \\                                          
                                 & \Data      &    {Data packet to satisfy a request}                              & \Data             & {Data packet to satisfy a request by an \Interest or \AddQInterest}                                                       \\  
                                 & -                         & -                                               & \DataStream       & {Data Stream packet representing continuous time series data}                          \\  
                                 & -                         & -                                               & \AddQInterest     & {Continuous Interest packet to express a continuous interest in the data object}                          \\  
                                 & -                         & -                                               & \RmQInterest      & {Remove Continuous Interest packet to remove interest on a data object}                         \\ \hline
\multirow{3}{*}{\begin{minipage}{2cm}Data Structures \\ (cf. \S\ref{subsubsec:components})\end{minipage}} & \ac{PIT} & Stores pending interests of consumer            & \ac{PIT}        & Stores pending interests and query interests                           \\  
                                 & \ac{CS}  & Stores data packets                             & \ac{CS}         & Stores dat
                                 a packets and buffers the data stream for stateful operators \\  
                                 & \ac{FIB} & Stores forwarding information towards producers & \ac{FIB}        & Stores forwarding information towards producers and consumers interested in CEP query                      \\ \hline
{\begin{minipage}{2cm}Data Processing  \\(cf. \S\ref{subsec:QE})  \end{minipage}}                & -                         & -                                               & \ac{CEP} engine & Parse, place, process and derive complex events                               \\ \hline
\end{tabular}
\setlength{\abovecaptionskip}{0pt}
\setlength{\belowcaptionskip}{-15pt}
\caption{\added{Description of differences in traditional \ac{ICN} vs \system architecture ("-" means no support).}}
%\vspace{-2mm}
\label{tab:differences}
\end{table*}

%We denote $l_{i,j}$ as the link interconnecting two brokers $b_i$ and $b_j$. . 
A producer multicasts the data stream (\DataStream packet) towards the broker network, which disseminates the stream through the network towards consumers that expressed their interest through \AddQInterest. 
%all over the network. The \DataStream packet is forwarded to further brokers in the network if there are consumers downstream for interested  in the data stream by means of an interest or a continuous interest.
%\emph{query interest} ($qi$). 
%An efficient event dissemination can be achieved by using routing algorithms, \eg defined in this work~\cite{Baldoni2007}, by looking at the similarity score of the \Interest.
%It also send a single \Data packet in response to an \Interest packet (pull).
%\circled{1} 
A consumer issues a query by sending an \Interest or an \AddQInterest packet comprising a query $q$ (top right \Cref{fig:inetcep}). Depending on the packet, the consumer receives the query result once or continuously. The \ac{CEP} query $q$ is processed by interconnected brokers forming a \emph{broker network}. %\circled{2} 
The query is stored in the \ac{PIT} just like the \Interest name on the receiving broker until %a \circled{3} 
\RmQInterest packet is received that triggers the removal of $q$ or \QInterest from the \ac{PIT} (bottom right \Cref{fig:inetcep}). 
%Unlike a conventional \ac{CEP} system, the event-based communication in the \system happens in the underlay CCN network.

The query $q$ induces a directed acyclic operator graph $G$% = (\Omega \cup P \cup C, D)$ ML: no need of definition?
, where a vertex is an operator $\omega \in \Omega$ and an edge represents the data flow of the data stream $D$. Each operator $\omega$ dictates a processing logic $f_\omega$. In the following, we explain the unified communication model, the operator graph and quality of information model.
 \newline
 

\textbf{Unified Communication Model.}\label{subsec:comm_model}
\added{The basic packet structure of a \ac{CCN} packet is shown in \Cref{fig:packet} that includes a fixed-size header whose size depends on the packet type, a variable length data object name, the optional name's TLV (type length value format), some optional TLVs and finally the payload. The maximum packet size of a CCN packet is 65KBytes, which is fragmented to fit the MTU of the communication protocol\footnote{For more information refer the IETF draft \url{https://tools.ietf.org/html/draft-ccn-packet-header-00}}.}
%The header comprises of versioning field to combine protocol version, the packet type (refer \Cref{tab:pak_types}), its length, hop limit used to limit the scope of the packet, flags to extend the fixed size header and finally the header length indicating the length of the hop by hop header. After the fixed size header, there are msg type and msg length fields same as pkt type and length for the reconstructed CCN packet to be self describing after fragmentation. The variable length name symbolizes the name prefix followed by the type length value format to encode variable length field like the name in CCN packets\footnote{For more information refer the IETF draft \url{https://tools.ietf.org/html/draft-ccn-packet-header-00}}.}

We provide five types of packets to support both kinds of interaction patterns. 
\Interest (\emph{request}) packet is equivalent to CCN's Interest packet that is used by the consumer to specify interest in the name of a data object or an operator ($\omega$). 
%\added{It comprises of a common fixed size header plus the msg type and msg length and TLV field. }
The \Data (\emph{reply}) packet is a \ac{CCN} data packet that satisfies an Interest or \AddQInterest detailed below. \added{This packet is similar to the \Interest with  additional payload that contains the content.}
%It also encapsulates the \emph{complex event} ($ce$) as described later.
The \DataStream packet represents a continuous time series data stream of the form $<ts, a_1, \ldots, a_m>$. 
Here, $ts$ is the time at which a tuple is generated and $a_i$ are the attributes of the tuple. \added{It is similar to the \Data packet in terms of structure except the packet type (refer \Cref{tab:pak_types}) and the payload comprising of the data stream.}
The \AddQInterest packet represents the interest in the form of a \ac{CEP} query $q$.  
\added{The structure is similar to \Interest packet and the query is encapsulated in the name.}
The \RmQInterest packet represents the \ac{CEP} query that should to be removed for the respective consumer (so that it no longer receives complex events).  %\added{This resembles the \AddQInterest packet in structure including the query in the name}.
The \ac{CCN} forwarding engine (data plane) is enhanced to handle these packets. We summarize the differences to classical \ac{ICN} architectures in \Cref{tab:differences}. 

\added{We model a flow from a CCN node as defined as a uni-directional data transfer from one node to another with feedback on the opposite direction on the same route. Flows are considered to be independent of each other and they can change dynamically. Furthermore packets in a flow are assumed to arrive in order (FIFO). }
\newline


\begin{figure}[t]

\begin{bytefield}[bitwidth=\linewidth/4, bitheight=12px]{4}
\bitheader[endianness=little]{0-3} \\
\bitbox{1}{\footnotesize Version} & \bitbox{1}{\footnotesize Pkt Type} & \bitbox{2}{\footnotesize Pkt Length}\\
\bitbox{1}{\footnotesize Hop Limit} & \bitbox{1}{\footnotesize FLAGS} & \bitbox{2}{\footnotesize Hdr Length}\\
\bitbox{2}{\footnotesize Msg Type} & \bitbox{2}{\footnotesize Msg Length}\\
\wordbox{1}{\footnotesize Variable Length Name}\\
\wordbox{1}{\footnotesize Optional Name TLVs}\\
\wordbox{1}{\footnotesize Optional Interest TLVs}\\
\wordbox{1}{\footnotesize Payload }\\
%\wordbox[lrb]{1}{}\\
\end{bytefield}
\caption{\added{\ac{CCN} packet structure.}}
\label{fig:packet}
\end{figure}


\begin{comment}

\textbf{Query Model.} \label{subsec:query_model}
We propose an expressive \ac{CEP} query language that can specify standard CEP operators and compose meaningful queries over the \ac{CCN} data plane. Although many \ac{CEP} query languages exist~\cite{Carbone2015ApacheFS}, our work differs from them in two ways:
%\begin{inparaenum}
	 they can handle only push-initiated interaction and function on IP in an overlay network, and
	 they are decoupled from the forwarding decisions taking place in the underlay (IP), which is not true in our approach.  
%\end{inparaenum}
The \system query language is based on two main design goals: 
%\begin{inparaenum}
    it should deal with both pull (data from relations) and push (time series data streams) kind of traffic, and
    support standard \ac{CEP} operators~%\TODO{give ref}
  (as identified in Section \ref{subsec:CEP}) over the \ac{CCN} data plane.
%\end{inparaenum}

Thus, a query ($q$) must be able to 
%\begin{inparaenum}
   capture time series data streams as well as relations of the form $<ts, a_1, .., a_m>$ and 
   define an operator $\omega$ with processing logic $f_\omega$ in a way that it is extensible. 
%\end{inparaenum}
\newline

\textbf{Operator Graph Model.} \label{subsec:op_model}
The operator graph $G$ is a directed acyclic graph of \emph{plan nodes}. The vertex of the graph is a plan node that encapsulates a single operator ($\omega$), while the links between plan nodes represents the data flow from the bottom of the graph to the top. The operator graph can be processed centrally or collaboratively in a distributed manner by mapping it to the underlay \ac{CCN} network. 
In distributed \ac{CEP}, typically, an operator placement mechanism defines a mapping of an operator graph $G$ onto a set of brokers, to collaboratively process the query. The placement needs to be coordinated with the forwarding decisions for efficient and parallel processing over the \ac{CCN} data plane.% defined as follows:
 One or more operators can be collocated on one broker depending on its capacity. 
\newline

\end{comment}

\added{\textbf{Quality of Information Model.}
One of the main objectives while unifying the communication strategies of ICN, is to minimize the delivery response time of the complex events, while maintaining high throughput of events.
% Short response times are extremely important for IoT applications such as in the prediction of high load in smart grid.
On top of that, there must not be any drop of events when delivering with short response time, which might result in wrong results.
We measure the drop of events or \textit{loss rate} in forwarding as $\frac{(\texttt{total events} - \texttt{processed events})}{\texttt{total events}}$.
%\rh{the windows operator reduces the number of events received even without any loss this formula would drop, right?} % \times 100$. 
Here, \texttt{total events} is the number of events that were produced by the producers and should have been received at the consumers end.
\texttt{Processed events} is the number of events that were eventually received at the consumer under the assumption that no operation in between intentionally reduces the number of events (cf. filter or windows).

To measure the correctness in the delivery of complex events while guaranteeing in-order processing, we refer to the \emph{accuracy} metric.
It is defined as the proximity of the derived complex events to the true complex events as a result of false positives and false negatives.
As a consequence of event drops, the derived complex events could be false positives or false negatives.
On the one hand, a false positive (FP) is defined as a complex event that should have been derived but is not or is falsely derived, while a false negative (FN) is an complex event that is derived when it should not have been derived.
Within our smart plug example, a false positive is a wrong prediction value as consequence of a drop in primitive events while a false negative is a missed prediction value when there should have been a prediction value generated.
On the other hand, the true positives (TP) and true negatives (TN) are correctly derived complex events, i.e., correct load predictions and not detected, respectively.
%Formally, the accuracy is defined as $\frac{TP + TN}{TP + TN + FP + FN}$.

In the following, we present the unified communication approach in~\Cref{subsec:unified} and the CEP query engine in~\Cref{subsec:QE}.}
\begin{comment} 

\added{\textbf{IoT Resource Model.}
Although we are restricted to a specific network topology and resource model, in \system we will focus on the resources commonly considered in the context of IoT applications. Consider a hierarchical tree-like infrastructure illustrated in \ml{todo figure} comprising of \emph{things} referring to IoT devices, a fixed network layer comprising of distributed sources in data centers or cloud, and an intermediate layer of resources at edge comprising of CCN routers. The cloud, edge and \emph{things} are assumed to communicate over CCN protocol as described in the system and communication model above. Here, \emph{things} represent data producers that generate continuous time-varying data stream. The consumer can be anywhere in the hierarchy while the brokers are represented by the edge, cloud and some of the devices in the things.}
\newline

\added{\textbf{QoS Model.}
An important principle of a CEP system is to satisfy an objective function of QoS demands, e.g., response time, bandwidth, throughput etc. \system allows specification of one or more QoS demands (QoS), with a focus on response time, throughput and correctness of events as defined before in the problem statement.
}


%%%%%%% this text is not in the paper!!! %%%%%%%
% An efficient event dissemination can be achieved by using routing algorithms~\cite{Baldoni2007} (this is out of scope for our work).
% like (SIENA) (%{give ref to Efficient Publish/Subscribe Through aSelf-Organizing Broker Overlay and its Application to SIENA paper}).
% our focus is to enable our CEP middleware including query and event notifications on the CCN architecture. 
 %We support the standard CEP operator processing logic for stateless and stateful operators (cf. \S\ref{subsec:CEP}) in our operator model and allow composition using our query language.

%Based on the scale of the received queries, the producers and the consumers, the broker either processes the queries in a centralized manner (single handedly) or distributes the operator graph ($G$) in the broker network. For distribution and placement of operators, first there is a need of network monitoring, and second, a criteria to be considered for placement (cf. \S\ref{subsec:ogprocessing}).
% The distribution and operator placement  is an NP-complete problem (\TODO{cite for proof}). We provide various heuristics 
%\begin{inparaenum}
%\item optimal,
%\item random and 
%\item decentralized placement to deal with the placement and distribution problem.
%\end{inparaenum}

%The pull based traffic is handled in the same way as before (cf. \S\ref{subsec:CCN}), we further define how the push based traffic or event notifications are handled.
%In this section, we first motivate the need of \system for a post-disaster relief scenario \ml{refer Using ICN in disaster scenarios} followed by the \system 's system model.  
%\subsection{System Model}
 %uncomment research question? then we have to do so for remaining as well
% In this work we investigate, \emph{if it is feasible to develop a general CEP query language that complies with the above goals, targeting a CCN architecture?} 
%%%%%%% this text is not in the paper!!! %%%%%%%
\begin{figure}
	\centering
	\includegraphics[width=1.2\linewidth, trim=0mm 0mm 0mm 0mm, clip=true]{figures/model}
	\setlength{\belowcaptionskip}{-20pt}
	\caption{System Model}
	\label{fig:model}
\end{figure}
%In Figure~\ref{fig:basicmode}, we illustrate the structure of our system model. We assume the presence of \emph{data producers}: who generates continuous stream of data, \emph{data consumers}: who specify interest in an event and \emph{data routers} or brokers: who host one or more operators collectively dictating the logic to infer the event of interest for the \emph{data consumer}. 
%%%%%%% this text is not in the paper!!! %%%%%%%
We first discuss in the overall system model 
\begin{inparaenum}
\item what system entities are involved 
\item and show how a query can be requested and processed within our system while conforming the default CCN communication (pull-based traffic is still supported).
\end{inparaenum} 
We use an example heat map query from the above section to explain the system model. Afterwards, we elaborate on the communication, query and the operator graph model respectively. 
\TODO{give sub sections later}
%\subsection{\textsc{CEP over ICN} Model}
ML: no need of definition?
 \[\alpha: \Omega \times B \rightarrow \{0,1\}, s.t. \]
\[
\alpha_{i,j} = \begin{cases}

  1, & \mbox{if $\omega_i$ is placed on $b_j$} \\
  0, & \mbox{if $\omega_i$ is not placed on $b_j$} \\
\end{cases}
\]

%The problem of finding a suitable mapping of the operator graph is well known as \emph{placement problem}. Although, there exists many solutions to the placement problem~\cite{Lakshmanan2008,Schilling2011}, in this work, we deal with the placement problem for a \ac{CCN} architecture by: 
%\begin{inparaenum}
%    \item discovery of optimal or sub optimal placement path while forwarding query interest,
%    \item handling network discovery, and
%    \item realizing state-of-the-art placement heuristics and decentralized solutions~\cite{Bonfils2004} over CCN architecture.
%\end{inparaenum}
 
%    \textsc{CEP over ICN} model allows processing of the operator graph $G$ in a centralized as well as in a decentralized manner. The flexibility of control of processing facilitates 
\end{comment}

